LivePose: Online 3D Reconstruction from Monocular Video with Dynamic Camera Poses

Dense 3D reconstruction from RGB images traditionally assumes static camera pose estimates. This assumption has endured, even as recent works have increasingly focused on real-time methods for mobile devices. However, the assumption of a fixed pose for each image does not hold for online execution: poses from real-time SLAM are dynamic and may be updated following events such as bundle adjustment and loop closure. This has been addressed in the RGB-D setting, by de-integrating past views and re-integrating them with updated poses, but it remains largely untreated in the RGB-only setting. We formalize this problem to define the new task of dense online reconstruction from dynamically-posed images. To support further research, we introduce a dataset called LivePose containing the dynamic poses from a SLAM system running on ScanNet. We select three recent reconstruction systems and apply a framework based on de-integration to adapt each one to the dynamic-pose setting. In addition, we propose a novel, non-linear de-integration module that learns to remove stale scene content. We show that responding to pose updates is critical for high-quality reconstruction, and that our de-integration framework is an effective solution.

==> tbl/2d_metrics.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{small}
\begin{tabular}{l c r r r}
    \toprule
     Method & $\delta <$ 1.25 &  Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RMSE $\downarrow$ \\
     \hline
     DeepVideoMVS&&&& \\
     Atlas&&&& \\
     NeuralRecon&&&& \\
     \hline
     Ours (Atlas)&&&& \\
     Ours (NeuralRecon)&&&& \\
    \bottomrule
\end{tabular}
\end{small}
}
\end{center}
\caption{\textbf{2D evaluation.} We compute 2D metrics by rendering depth from mesh following Atlas \cite{atlas}.}
\label{tab:2d_metrics}
\end{table}

==> tbl/performance.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{small}
\begin{tabular}{l c r r r}
    \toprule
    
     \multirow{2}{*}[-0.3em]{Base method} & \multirow{2}{*}[-0.3em]{Strategy} & \multirow{2}{*}[-0.3em]{F-score$\uparrow$} &  \multicolumn{2}{c}{Latency (ms)} \\
     \cmidrule(lr){4-5}
      & & & \multicolumn{1}{c}{New} & \multicolumn{1}{c}{Update}\\
    \midrule
    \multirow{3}{*}[0.0em]{Atlas \cite{atlas}} & No updates & 0.531 & 2,481 & 0 \\
     & Re-integration & 0.545 & 2,492 & 2,363 \\
     & Ours & \textbf{0.564} & 2,475 & 2,673 \\
    \midrule[0.1pt]
    \multirow{3}{*}[0.0em]{NeuralRecon \cite{neuralrecon}} & No updates & 0.546 & 223 & 0 \\
     & Re-integration & 0.568 & 223 & 233 \\
     & Ours & \textbf{0.577} & 211 & 426 \\
    \midrule[0.1pt]
    \multirow{3}{*}[0.0em]{DeepVideoMVS \cite{deepvideomvs}} & No updates & 0.521 & 1,081 & 0 \\
     & Re-integration & 0.535 & 1,081 & 143 \\
     & Ours &\textbf{0.554} & 1,081 & 287 \\
    \bottomrule
\end{tabular}
\end{small}
}
\end{center}
\caption{\textbf{Performance.} With our learned de-integration module, NeuralRecon averages $223$ms to integrate a new bundle (9 keyframes) and 426ms to update a past bundle, which is tractable for interactive applications. We achieve significantly reduced update time for DeepVideoMVS by estimating the depth only once for each view, and re-using that same depth during de-/re-integration. }
\label{tab:performance}
\end{table}
